A Distributionally Robust Approach to Fair Classification

We propose a distributionally robust logistic regression model with an unfairness penalty that prevents discrimination with respect to sensitive attributes such as gender or ethnicity. This model is equivalent to a tractable convex optimization problem if a Wasserstein ball centered at the empirical distribution on the training data is used to model distributional uncertainty and if a new convex unfairness measure is used to incentivize equalized opportunities. We demonstrate that the resulting classifier improves fairness at a marginal loss of predictive accuracy on both synthetic and real datasets. We also derive linear programming-based confidence bounds on the level of unfairness of any pre-trained classifier by leveraging techniques from optimal uncertainty quantification over Wasserstein balls.

==> style2.tex <==
% ================== Margins & Layout =================================
\addtolength{\voffset}{0cm} 
\addtolength{\textheight}{1cm} 
\addtolength{\hoffset}{-2cm}
\addtolength{\textwidth}{4cm}

\setlength{\parskip}{1mm}
\linespread{1.12}

%======== Section numbering ===============================
\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{\thesection.\arabic{subsection}}

% ====== Change section title ===============================
\makeatletter
\def\@settitle{\begin{center}%
		\baselineskip14\p@\relax
		\normalfont\LARGE\scshape\bfseries
		%\uppercasenonmath\@title
		\@title
	\end{center}%
}
\makeatother
\makeatletter

\def\subsection{\@startsection{subsection}{2}%
	\z@{.5\linespacing\@plus.7\linespacing}{.5\linespacing}%
	{\normalfont\large\bfseries}}

\def\subsubsection{\@startsection{subsubsection}{3}%
	\z@{.5\linespacing\@plus.7\linespacing}{.5\linespacing}%
	{\normalfont\itshape}}

% ================== Packages =================================
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{dsfont, amssymb, amsmath, graphicx, enumitem, wrapfig, subcaption} %,etaremune,savesym}
\usepackage{amsfonts,dsfont,mathtools, mathrsfs, amsthm, accents} 
\usepackage[amssymb, thickqspace]{SIunits}
\usepackage{enumitem}


%================================ Theorem ======================================
\usepackage{amsthm}
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%===============================================================================

%================================ Packages =====================================
\usepackage[numbers]{natbib}
\usepackage{mathrsfs, mathtools, fancyhdr, cases}
\usepackage{float, color, bm, bbm}
\usepackage{graphicx, epstopdf, transparent} 
\usepackage{multirow, titlecaps, bigstrut}
\usepackage{algorithm, algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}
\usepackage[utf8]{inputenc}    % allow utf-8 input
\usepackage[T1]{fontenc}        % use 8-bit T1 fonts
\usepackage{lmodern}             % allow pdf compability
\usepackage{multirow}
\usepackage{wrapfig}


%============================== Abbreviation ===================================
\DeclareMathOperator{\Tr}{tr}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\bahar}[1]{\begin{tcolorbox}[width=\textwidth, colframe=purple, boxrule=0.5pt, boxsep=0.001mm]{{\footnotesize{Bahar: #1}}}\end{tcolorbox}}
\newcommand{\viet}[1]{\begin{tcolorbox}[width=\textwidth, colframe=blue
, boxrule=0.5pt, boxsep=0.001mm]{{\footnotesize{Viet: #1}}}\end{tcolorbox}}

\newcommand{\Pnom}{\hat \PP} 
\newcommand{\supp}{\textrm{supp}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}
\newcommand{\mbb}{\mathbb}
\newcommand{\Wass}{\mathds W}
\newcommand{\VV}{\mathds V}
\newcommand{\opt}{^\star}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle }
\newcommand{\ds}{\displaystyle}

\newcommand{\defeq}{\coloneqq}
\newcommand{\pd}{\mathbbm{P}}
\newcommand{\ie}{\textit{i.e., }}
\newcommand{\R}{\mathbb{R}}
\newcommand{\wh}{\hat}
\newcommand{\dist}{\textrm{\textbf{dist}}}
\newcommand{\mc}{\mathcal}
\newcommand{\m}{\mathcal{M}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\x}{\mathcal{X}}
\newcommand{\y}{\mathcal{Y}}
\newcommand{\asinh}{\textrm{arcsinh}}
\newcommand{\samplerate}{\mathcal{O}}
\newcommand{\cdf}{F}
\newcommand{\bs}{\boldsymbol}
\newcommand{\ctransj}{\dvy_j-c(x,y_j)}
\newcommand{\ctransjneg}{-\dvy_j+c(x,y_j)}
\newcommand{\euler}{\gamma}
\newcommand{\DS}{\displaystyle}
\newcommand{\st}{\mathrm{s.t.}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eps}{\varepsilon}

